CRoW: Benchmarking Commonsense Reasoning in Real-World Tasks

Recent efforts in natural language processing (NLP) commonsense reasoning research have yielded a considerable number of new datasets and benchmarks. However, most of these datasets formulate commonsense reasoning challenges in artificial scenarios that are not reflective of the tasks which real-world NLP systems are designed to solve. In this work, we present CRoW, a manually-curated, multi-task benchmark that evaluates the ability of models to apply commonsense reasoning in the context of six real-world NLP tasks. CRoW is constructed using a multi-stage data collection pipeline that rewrites examples from existing datasets using commonsense-violating perturbations. We use CRoW to study how NLP systems perform across different dimensions of commonsense knowledge, such as physical, temporal, and social reasoning. We find a significant performance gap when NLP systems are evaluated on CRoW compared to humans, showcasing that commonsense reasoning is far from being solved in real-world task settings. We make our dataset and leaderboard available to the research community at https://github.com/mismayil/crow.

==> temp0.3-0.5-results-table.tex <==

\begin{table*}[t!]
\footnotesize
\centering
\scalebox{0.72}{
\begin{tabular}{lrrrrrrrrrrr}
\toprule
   \multirow{2}{*}{\textbf{Models}}
 & \multicolumn{4}{c}{{\textbf{MT}}} 
 & \multicolumn{1}{c}{{\textbf{DG}}}
 & \multicolumn{1}{c}{{\textbf{DS}}}
 & \multicolumn{1}{c}{{\textbf{SC}}}
 & \multicolumn{1}{c}{{\textbf{SD}}}
 & \multicolumn{1}{c}{{\textbf{ID}}}
 & \multicolumn{1}{c}{{\textbf{CROW}}}
 & \multicolumn{1}{c}{{\textbf{CROW}}}  \\
 
 & \multicolumn{1}{c}{Zh-En}& \multicolumn{1}{c}{En-Fr}  & \multicolumn{1}{c}{En-De} & \multicolumn{1}{c}{En-Ru} & & & & & & \multicolumn{1}{c}{\textbf{Score (-MT)}} & \multicolumn{1}{c}{\textbf{Score}} \\
 \midrule
\textbf{Majority} & 33.3 / 0.0 & 33.3 / 0.0 & 33.3 / 0.0 & 33.3 / 0.0 & 40.1 / 0.0 & 42.8 / 0.0 & 33.6 / 0.0 & 36.5 / 0.0 & 41.3 / 0.0 & 38.9 / 0.0 & 36.4 / 0.0 \\
\textbf{Random} & 49.9 / 25.4 & 50.0 / 24.7 & 50.3 / 24.9 & 49.0 / 23.8 & 48.1 / 14.4 & 46.4 / 9.9 & 50.6 / 6.9 & 49.8 / 0.6 & 48.3 / 10.2 & 48.6 / 8.4 & 49.1 / 15.6 \\
\midrule
\textbf{LLaMa-7B} & 33.4 / 0.2 & -- & -- & -- & 51.0 / 8.7 & 49.5 / 7.4 & 33.7 / 0.3 & 29.9 / 0.0 & 41.3 / 0.0 & 41.1 / 3.3 & 39.8 / 2.7 \\
\textbf{LLaMa-13B} & 48.0 / 17.7 & -- & -- & -- & 50.6 / 12.9 & 50.6 / 9.2 & 39.2 / 3.6 & 35.3 / 0.1 & 50.2 / 7.7 & 45.2 / 6.7 & 45.7 / 8.5 \\
\textbf{LLaMa-33B} & 33.4 / 0.2 & -- & -- & -- & 54.6 / 9.9 & 53.5 / 9.5 & 33.7 / 0.3 & 31.7 / 0.1 & 42.8 / 1.0 & 43.2 / 4.1 & 41.6 / 3.5 \\
\textbf{Flan-T5-11B} & 56.7 / 29.3 & -- & -- & -- & \hl{66.6 / 36.2} & \hl{65.0 / 29.9} & \hl{74.7 / 45.2} & \hl{81.5 / 27.5} & \hl{81.6 / 53.5} & \hl{73.9 / 38.4} & \hl{71.0 / 36.9} \\
\textbf{Alpaca} & 41.0 / 7.5 & -- & -- & -- & 54.4 / 16.7 & 54.5 / 11.7 & 41.5 / 6.4 & 45.5 / 2.4 & 52.9 / 10.1 & 49.8 / 9.4 & 48.3 / 9.1 \\
\textbf{Flan-Alpaca} & 60.2 / 28.4 & -- & -- & -- & 61.1 / 26.9 & 52.3 / 18.4 & 67.0 / 35.7 & 66.3 / 9.5 & 78.0 / 45.1 & 65.0 / 27.1 & 64.2 / 27.3 \\
\textbf{Vicuna} & 41.7 / 8.7 & -- & -- & -- & 59.8 / 21.6 & 59.0 / 17.5 & 45.6 / 11.6 & 42.6 / 0.8 & 57.3 / 14.9 & 52.9 / 13.3 & 51.0 / 12.5 \\
\textbf{Stable-Vicuna} & 58.0 / 28.4 & -- & -- & -- & 52.5 / 13.6 & 41.4 / 7.7 & 51.3 / 16.4 & 66.9 / 11.8 & 61.9 / 21.7 & 54.8 / 14.2 & 55.3 / 16.6 \\
\midrule
\textbf{mT0} & 54.6 / 22.6 & 40.5 / 7.3 & 38.2 / 4.5 & 34.5 / 1.3 & 46.6 / 7.2 & 53.6 / 11.9 & 57.2 / 16.0 & 55.5 / 2.6 & 53.4 / 10.7 & 53.2 / 9.7 & 48.2 / 9.4 \\
\textbf{BloomZ-7B} & 53.9 / 21.8 & 49.9 / 20.0 & 49.9 / 19.9 & 50.3 / 20.5 & 54.4 / 15.9 & 53.6 / 14.2 & 57.2 / 13.9 & 64.4 / 6.1 & 60.5 / 20.4 & 58.0 / 14.1 & 54.9 / 17.0 \\
\midrule
\textbf{PaLM 1} & 33.8 / 0.6 & 34.2 / 1.1 & 34.1 / 0.9 & 33.4 / 0.3 & 63.6 / 26.8 & 62.6 / 23.0 & 51.6 / 15.4 & 56.6 / 7.9 & 63.5 / 21.9 & 59.6 / 19.0 & 48.2 / 10.9 \\
\textbf{GPT-3} & 66.7 / 39.4 & 48.5 / 16.1 & 49.2 / 17.2 & 48.1 / 12.1 & 67.1 / 36.8 & 68.6 / 32.6 & 69.2 / 38.2 & 85.6 / 39.5 & 76.4 / 42.0 & 73.4 / 37.8 & 64.2 / 29.7 \\
\textbf{GPT-4} & \hl{75.6 / 56.6} & 54.5 / 22.1 & 54.6 / 20.3 & 53.8 / 20.5 & \hl{72.0 / 45.6} & \hl{90.5 / 77.3} & 81.5 / 57.3 & \hl{89.2 / 50.2} & \hl{84.7 / 59.0} & \hl{83.6 / 57.9} & \hl{72.9 / 45.4} \\
\textbf{GPT-4-CoT} & 71.2 / 51.1 & \hl{64.3 / 41.9} & \hl{57.5 / 34.3} & \hl{56.9 / 29.2} & 55.2 / 23.1 & 89.0 / 71.7 & \hl{83.6 / 60.6} & 88.2 / 47.0 & 84.2 / 57.8 & 80.0 / 52.0 & 72.2 / 46.3 \\

\midrule 
\textbf{Human$^*$}   &  87.9  /  78.0  & 83.0  /  82.9  &  89.9  /  82.0 & 89.9  /  86.0  &  87.0  /  86.9 & 98.9  /  96.4 & 88.1  /  69.6 & 97.8  /  93.9 & 93.9  /  80.7 & 93.1  /  85.5  & 90.7  /  84.0 \\
\bottomrule
\end{tabular}}
\caption{\textbf{Macro-F1} / \textbf{Situational Accuracy} (\ie, results aggregated per \textit{context} instead of per \textit{sample}) for all examined models across \ourbenchmark{} tasks. \mete{All model results are averaged over three runs with different seeds.} $^*$Due to the cost of expert evaluation, our \textbf{Human} study is only evaluated on 100 instances per task.}
\label{tab:main_results}
\end{table*}
